Diagonally-Weighted Generalized Method of Moments Estimation for Gaussian Mixture Modeling

With direct computation of moments through order $L$ in $d$ dimensions, standard method of moments (MM) incurs $\Omega(d^L)$ computation and storage costs, and standard generalized method of moments (GMM) additionally requires estimating and inverting an often ill-conditioned covariance matrix of size $\Omega(d^L)$-by-$\Omega(d^L)$ to obtain the optimal weighting matrix. Pereira, Kileel, and Kolda [arXiv:2202.06930 (2022)] avoid the tensor computation cost of MM through implicit moment computation. Despite this progress, incorporating statistically principled weighting while preserving computational efficiency remains an important challenge, particularly at low signal-to-noise ratio (SNR), where sampling variances can differ substantially across moment orders. We introduce diagonally-weighted GMM (DGMM), which assigns one adaptive weight to each moment order through a structured approximation of the optimal weighting matrix while avoiding the covariance inversion, thereby balancing statistical efficiency, computational complexity, and numerical stability. For general parametric models, we prove that DGMM is consistent, asymptotically normal, and near-efficient under explicit structural conditions. For heteroscedastic low-rank Gaussian mixtures, we design a computationally efficient and numerically stable algorithm that extends the implicit moment computation to the DGMM objective, gradients, and weights and incorporates Nystr\"om approximations of the kernel sums. In low-SNR experiments with $d=100$ and $L=4$, where standard MM and GMM are infeasible, controlled weighting comparisons show that DGMM achieves consistently small parameter errors across tested initializations, including the challenging starts where alternative weightings struggle, with shorter median runtimes and fewer iterations. The code and data will be available upon publication at https://github.com/liu-lzhang/dgmm.

==> dgmm_arxiv-pratenddefaultcategory.tex <==


\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndii}]\phantomsection\label{proof:prAtEndii}Define the \emph {population objective function}: \begin {align} Q(\btheta ) \coloneq \EX \left [g\left ({\btheta }; \by _n \right )\right ]^\top W \EX \left [g\left ({\btheta }; \by _n \right )\right ], \mkern 9mu W = \diag (\underbrace {w_1, \dots , w_1}_{d \text { copies}}, \dots , \underbrace {w_L, \dots , w_L}_{d^L \text { copies}}). \end {align} \par We check the standard regularity conditions for consistency, in e.g.~\cite [Theorem~2.6]{newey1994large}: \begin {enumerate}[label=(\alph *)] \item The sample data is \text {i.i.d.}, assumed in the specifications of \cref {model:heteroscedastic}. \item The parameter space $\Theta $ is compact and contains $\btheta ^\star $ as an interior point, which is a standard assumption. \item The moment function $g(\btheta ; \by _n)$ in \cref {eq:moment-function} depends polynomially on the parameter $\btheta $ and is therefore continuous at each $\btheta \in \Theta $. \item Since $\Theta $ is compact and all moments of any finite Gaussian mixture are finite, we have $\EX [\sup _{\btheta \in \Theta } \norm {g(\btheta ; \by _n)}]< \infty $. \item The model is globally identifiable, which is a standard assumption (see \Cref {sec:mm-gmm}). \item The DGMM weighting matrices in \cref {eq:d-gmom-multistep} satisfy $\widehat {W}^{[t]} \xrightarrow {p} W$. $W$ is positive-definite due to the following: The numerator in \cref {eq:d-gmom-multistep} $\Tr \left [S^{(k,k)}\right ] = \EX [\norm {g^{(k)}(\btheta ^\star ; \by _n)}^2 ] > 0$. The denominator in \cref {eq:d-gmom-multistep} is positive: every term under the double sum is a square, with at least one strictly positive entry. \end {enumerate} \par Therefore, we get that ${\widehat {\btheta }}^{[t]}\xrightarrow {p} \btheta ^\star $, which proves the consistency of ${\widehat {\btheta }}^{(\dgmm )}$. \par To show that ${\widehat {\btheta }}^{(\dgmm )}$ is asymptotically normal, in addition to the above regularity conditions for consistency, we need to check the following conditions: \begin {enumerate}[label=(\alph *), resume] \item The moment function $g(\btheta ; \by _n)$ in \cref {eq:moment-function} is continuously differentiable in a neighborhood of $\btheta ^\star $ with probability approaching one as $N\to \infty $. \item $\EX [\norm {g(\btheta ^\star ; \by _n)}^2] < \infty $ and $\EX [\sup _{\btheta \in \cN (\btheta ^\star )} \norm {\nabla _{\btheta } g(\btheta ; \by _n)}]< \infty $, which follows from the definitions of \cref {model:heteroscedastic} and \cref {eq:moment-function}. \item $G(\btheta ^\star )^\top W G(\btheta ^\star )$ is non-singular, which follows from the fact that $W$ is positive-definite and the standard assumption discussed in \Cref {sec:mm-gmm} that the model is locally identifiable, that is, $\rank (G(\btheta ^\star )) = p$. \end {enumerate} \par By the standard asymptotic normality result, in e.g.~\cite [Theorem~3.4]{newey1994large}, if conditions (a)-(i) are satisfied, then for any GMM estimator $\widehat {\btheta }$, \begin {align} \sqrt {N} \left (\widehat {\btheta } - \btheta ^\star \right ) \xrightarrow {d} \cN \left (\bm {0}, \left (G^\top W G\right )^{-1} G^\top W S W G \left (G^\top W G\right )^{-1} \right ), \end {align} where we write $G = G(\btheta ^\star )$ for notational convenience. For the DGMM estimator, since the weighting matrix $W$ is block-diagonal, we can express the asymptotic variance $S$ in block form to highlight how each moment group contributes to the overall asymptotic variance. To do this, we partition the Jacobian matrix $G$ into $L$ blocks, $G = \left [{G^{(1)}}^\top ,\dots ,{G^{(L)}}^\top \right ]^\top $, so that ${G^{(k)}}$ is the $d^k$-by-$p$ submatrix of $G$ corresponding to the $k$-th moment. We also partition $S$ into blocks such that $S^{(k, k^\prime )}$ is the $d^k$-by-$d^{k^\prime }$ submatrix of $S$, consisting of the cross-order covariance between the $k$-th and $k^\prime $-th sample moment conditions, for $k, k^\prime = 1, \dots , L$, i.e., \begin {align} S^{(k, k^\prime )} \coloneq \left (S_{ij}\right )_{i\in \cI _k, j\in \cI _{k^\prime }} = \EX \left [ g^{(k)}(\btheta ^\star ; \by _n) g^{(k^\prime )}(\btheta ^\star ; \by _n)^\top \right ]. \end {align} Then we get the form of the asymptotic covariance matrix of $\widehat {\btheta }^{(\dgmm )}$ in \cref {eq:dgmm-asymptotic-efficiency}.\end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiii}]\phantomsection\label{proof:prAtEndiii}\par As shown in \cite [Theorem~3.2]{hansen1982large}, in the class of GMM estimators, $V^{(\gmm )} = \left (G^\top S^{-1} G\right )^{-1}$ is the minimum asymptotic covariance within the class of GMM estimators, which directly implies that $V^{(\dgmm )} -V^{(\gmm )} \succeq 0$. We now obtain the upper bound on $V^{(\dgmm )}$. Let $W$ be the DGMM weighting matrix in \cref {eq:w_k-direct}. We first apply a change of coordinate to get $\widetilde {S} = W^{\frac {1}{2}} S W^{\frac {1}{2}}$. Let $E = \widetilde {S} - I_q$. Then \begin {align} E^{(k, k)} = w_k S^{(k,k)} - I_{d^k}, \quad E^{(k, k^\prime )} = \sqrt {w_k w_{k^\prime }} S^{(k, k^\prime )} (k\neq k^\prime ). \end {align} Since $E$ is a symmetric matrix, $E^{(k, k^\prime )} = {E^{(k^\prime , k)}}^\top $ and so $\normop {E^{(k, k^\prime )}} = \normop {E^{(k^\prime , k)}}$. For an arbitrary vector $\bx = \left [\bx _1; \cdots ; \bx _L \right ] \in \R ^q$ where $\bx _k \in \R ^{d^k}$, by applying Cauchy-Schwarz, AM-GM inequality, and the symmetry of $E$, we get \begin {align*} |\bx ^\top E \bx | \leq \sum _{k, k^\prime } \normop {E^{(k, k^\prime )}} \norm {\bx _k} \norm {\bx _{k^\prime }} &\leq \frac {1}{2} \sum _{k, k^\prime } \normop {E^{(k, k^\prime )}} \left ( \norm {\bx _k}^2 + \norm {\bx _{k^\prime }}^2 \right ) \\ &= \sum _{k} \left ( \sum _{k^\prime } \normop {E^{(k, k^\prime )}} \right ) \norm {\bx _k}^2 \leq \eta \norm {\bx }^2, \end {align*} where the last step is due to \cref {eq:near-efficiency-condition}. So we get $(1- \eta ) I_q \preceq \widetilde {S} \preceq (1+\eta ) I_q$, which implies that for any eigenvalue $\lambda $ of $\widetilde {S}$, $\lambda \in [1- \eta , 1+ \eta ]$ and is strictly positive. Therefore, \begin {align} (\lambda - (1- \eta )) ((1+\eta ) - \lambda ) \geq 0 \implies \lambda + \frac {1-\eta ^2}{\lambda } \leq 2 \implies \widetilde {S} + (1-\eta ^2) \widetilde {S}^{-1} \preceq 2 I_q. \label {eq:eta-bound-Stilde} \end {align} Define $\widetilde {G} = W^{\frac {1}{2}} G$. Substituting $G = W^{- \frac {1}{2}} \widetilde {G} $ and $S^{-1} = W^{\frac {1}{2}} \widetilde {S}^{-1} W^{\frac {1}{2}}$ into the asymptotic covariances $V^{(\dgmm )} = \left (G^\top W G\right )^{-1} G^\top WSWG \left (G^\top W G\right )^{-1}, V^{(\gmm )} = \left (G^\top S^{-1} G\right )^{-1}$: \begin {align} V^{(\dgmm )} = \left (\widetilde {G}^\top \widetilde {G} \right )^{-1} \widetilde {G}^\top \widetilde {S} \widetilde {G} \left (\widetilde {G}^\top \widetilde {G} \right )^{-1}, \quad V^{(\gmm )} = \left (\widetilde {G}^\top \widetilde {S}^{-1} \widetilde {G} \right )^{-1}. \label {eq:change-of-coord-variance} \end {align} \par By combining \cref {eq:eta-bound-Stilde} and \cref {eq:change-of-coord-variance} and using the shorthand $ H \coloneq \left (\widetilde {G}^\top \widetilde {G} \right )^{-1} $, we get \begin {align*} H \widetilde {G}^\top \left ( \widetilde {S} + (1-\eta ^2) \widetilde {S}^{-1} \right )\widetilde {G} H &\preceq H \widetilde {G}^\top \left ( 2 I_q\right ) \widetilde {G} H \\ V^{(\dgmm )} + (1-\eta ^2) H \left (V^{(\gmm )} \right )^{-1} H &\preceq 2 H \\ V^{(\dgmm )} & \preceq 2 H - (1-\eta ^2) H \left (V^{(\gmm )} \right )^{-1} H . \numberthis \label {eq:upper-bound-step} \end {align*} \par By a completion-of-the-square argument inspired by the proof of \cite [Theorem 3.2]{hansen1982large}, we get \begin {align*} &\frac {1}{1-\eta ^2} V^{(\gmm )} - \left ( 2 H - (1- \eta ^2) H \left (V^{(\gmm )} \right )^{-1} H \right ) \\ =& (1- \eta ^2) \left ( H - \frac {1}{1-\eta ^2} V^{(\gmm )} \right ) \left (V^{(\gmm )} \right )^{-1} \left ( H - \frac {1}{1-\eta ^2} V^{(\gmm )} \right ) \succeq 0, \end {align*} where the last step is due to $\left (V^{(\gmm )} \right )^{-1} \succ 0, 1-\eta ^2 >0$. It then follows that \begin {align} 2 H - (1- \eta ^2)H \left (V^{(\gmm )} \right )^{-1} H \preceq \frac {1}{1-\eta ^2} V^{(\gmm )}.\label {eq:complete-the-square-step} \end {align} \par Combining \cref {eq:upper-bound-step} and \cref {eq:complete-the-square-step}, we get $V^{(\dgmm )} \preceq \frac {1}{1-\eta ^2} V^{(\gmm )} = \left (1 + \frac {\eta ^2}{1- \eta ^2}\right ) V^{(\gmm )}.$ \par \end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndiv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofiv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndiv}]\phantomsection\label{proof:prAtEndiv}\label {pf:computational-complexity-norm} We compute $\phi ^{(k)} (\btheta )$ by applying \cref {prop:mom-cum-bell}: \begin {align*}\label {eq:F_1} \phi ^{(k)} (\btheta ) &= \sum _{i=1}^K \sum _{j=1}^K \pi _i \pi _j \left \langle \cM ^{(k)}({\btheta }_i), \cM ^{(k)}({\btheta }_j)\right \rangle = \sum _{i=1}^K \sum _{j=1}^K \pi _i \pi _j B_k\left (\kappa ^{(1)}_{ij} , \dots , \kappa ^{(k)}_{ij} \right ) \numberthis , \end {align*} where $\cM ^{(k)}({\btheta }_j)$ denotes the $k$-th moment of the $j$-th Gaussian component, ${\btheta }_j = \left [\pi _j; {\bmu }_j ; V_j \right ]^\top $ are the parameters of the $j$-th Gaussian component, and $\kappa ^{(l)}_{ij}$ denotes the $l$-th cumulant of the inner product between the $i$-th Gaussian component ${\bX }_i$ and an independent draw of the $j$-th Gaussian component ${\bX }_j^\prime $, i.e., $\kappa ^{(l)}_{ij} \coloneq \kappa ^{(l)}\left (\inner {{\bX }_i}{{\bX }_j^\prime }\right ), l = 1, \dots , k$. The Bell polynomials are evaluated by applying the recurrence relation (see, e.g., \cite [Theorem~11.2]{charalambides2018enumerative} or \cite [Eq.~7.12]{bell1934exponential}): \begin {align} \label {eq:alpha-recurrence} \begin {cases*} B_0 = 1, & (base case)\\ B_{k}\left ( \kappa ^{(1)}_{ij}, \dots , \kappa ^{(k)}_{ij} \right ) = \sum _{l=0}^{k-1} {k-1 \choose l}B_{k-l-1}\left (\kappa ^{(1)}_{ij}, \dots , \kappa ^{(k-l-1)}_{ij}\right ) \kappa ^{(l+1)}_{ij}. & (induction step) \end {cases*} \end {align} By applying \cite [Proposition 3.3]{pereira2022tensor}, \begin {align} \label {eq:cumulants} \kappa ^{(l)}_{ij} = \begin {cases*} \left \langle {\bmu }_j, {\bmu }_i \right \rangle , & ($l = 1$) \\ (l-1)! \Tr ((V_i {V_i}^\top V_j {V_j}^\top )^{\frac {l}{2}}) + \frac {l!}{2} {{\bmu }_i}^\top V_j {V_j}^\top (V_i {V_i}^\top V_j {V_j}^\top )^{\frac {l-2}{2}} {\bmu }_i \\ \quad + \frac {l!}{2} {{\bmu }_j}^\top (V_i {V_i}^\top V_j {V_j}^\top )^{\frac {l-2}{2}}V_i {V_i}^\top {\bmu }_j, & ($l$ is even) \\ l! {{\bmu }_j}^\top (V_i {V_i}^\top V_j {V_j}^\top )^{\frac {l-1}{2}} {\bmu }_i. & ($l$ is odd) \\ \end {cases*} \end {align} Note that the computational complexity of the matrix multiplication $V_j^\top V_j$ is $\cO (d R_j^2)$, better than that of $V_j V_j^\top $, which is $\cO (d^2R_j)$. By carefully choosing the order of the consecutive matrix multiplication, we compute $\kappa ^{(l)}_{ij}$ in \cref {eq:cumulants} using $\cO (ldR_{\max }^2)$ operations\footnote {Our implementation also follows this faster order.}. $\phi ^{(k)} (\btheta )$ in \cref {eq:F_1} requires (1) pre-computing $\kappa ^{(l)}_{ij}$ for all $i,j \in [K]$ and $l\in [k]$ in $\cO (k K^2 d R_{\max }^2)$ operations, (2) using the recurrence relation in \cref {eq:alpha-recurrence} to compute $B_{k}\left ( \kappa ^{(1)}_{ij}, \dots , \kappa ^{(k)}_{ij} \right )$ for all $i,j \in [K]$ in $\cO (k^2 K^2)$ operations. In total, $\phi ^{(k)} (\btheta )$ takes $\cO (k^2 K^2 + k K^2 d R_{\max }^2)$ operations. \par The derivative of the Bell polynomials is given by {\cite [Eq. 5.1]{bell1934exponential}}: \begin {equation} \frac {\partial B_k}{\partial x_i}(x_1, \dots , x_k) = \binom {k}{i} B_{k-i} (x_1, \dots , x_{k-i}). \end {equation} Using \cref {eq:F_1}, the above identity, and the chain rule, we compute: \begin {align*} \nabla _{\pi _j} \phi ^{(k)} (\btheta ) &= 2 \sum _{i=1}^K \pi _i B_{k} \left (\kappa ^{(1)}_{ij},\dots , \kappa ^{(k)}_{ij}\right ),\numberthis \\ \nabla _{{\bmu }_j}\phi ^{(k)} (\btheta ) &= 2 \sum _{i=1}^K \pi _i \pi _j \sum _{l=1}^k \binom {k}{l} B_{k-l} \left (\kappa ^{(1)}_{ij},\dots , \kappa ^{(k-l)}_{ij}\right ) \nabla _{{\bmu }_j} \kappa ^{(l)}_{ij},\numberthis \\ \nabla _{V_j} \phi ^{(k)} (\btheta ) &= 2 \sum _{i=1}^K \pi _i \pi _j \sum _{l=1}^k \binom {k}{l} B_{k-l} \left (\kappa ^{(1)}_{ij},\dots , \kappa ^{(k-l)}_{ij}\right ) \nabla _{V_j} \kappa ^{(l)}_{ij}.\numberthis \end {align*} From the cumulants in \cref {eq:cumulants}, we get the gradients of the cumulants w.r.t.~${\bmu }_j$ and $V_j$: \begin {equation} \label {eq:cumulants-gradients-mu} \nabla _{{\bmu }_j} \kappa ^{(l)}_{ij} = \begin {cases*} {\bmu }_i , & ($l = 1$) \\ l! \left (V_i {V_i}^\top V_j {V_j}^\top \right )^{\frac {l-2}{2}} V_i {V_i}^\top {\bmu }_j, & ($l$ is even) \\ l! \left (V_i {V_i}^\top V_j {V_j}^\top \right )^{\frac {l-1}{2}} {\bmu }_i, & ($l$ is odd) \\ \end {cases*} \end {equation} \begin {align} \label {eq:cumulants-gradients-v} \nabla _{V_j} \kappa ^{(l)}_{ij} &= \begin {cases*} 0 , & ($l = 1$) \\ l! \left (V_i {V_i}^\top V_j {V_j}^\top \right )^{\frac {l-2}{2}} V_i {V_i}^\top V_j \\ \quad + l! \sum _{p=0}^{\frac {l-2}{2}} \left (V_i {V_i}^\top V_j {V_j}^\top \right )^p {\bmu }_i {{\bmu }_i}^\top \left (V_j {V_j}^\top V_i {V_i}^\top \right )^{\frac {l-2}{2} - p} V_j \\ \quad + l! \sum _{p=0}^{\frac {l-2}{2}-1} V_i {V_i}^\top \left (V_j {V_j}^\top V_i {V_i}^\top \right )^p {\bmu }_j {{\bmu }_j}^\top \left (V_i {V_i}^\top V_j {V_j}^\top \right )^{\frac {l-2}{2}-1 - p} V_i {V_i}^\top V_j, & ($l$ is even) \\ l! \sum _{p=0}^{\frac {l-1}{2}-1} V_i {V_i}^\top \left (V_j {V_j}^\top V_i {V_i}^\top \right )^p {\bmu }_j {{\bmu }_i}^\top \left (V_j {V_j}^\top V_i {V_i}^\top \right )^{\frac {l-1}{2}-1-p} V_j \\ \quad + l! \sum _{p=0}^{\frac {l-1}{2}-1} \left (V_i {V_i}^\top V_j {V_j}^\top \right )^p {\bmu }_i {{\bmu }_j}^\top \left (V_i {V_i}^\top V_j {V_j}^\top \right )^{\frac {l-1}{2}-1-p} V_i {V_i}^\top V_j. & ($l$ is odd) \end {cases*} \end {align} $\nabla _{\pi _j}\phi ^{(k)} (\btheta )$ requires (1) pre-computing $\kappa ^{(l)}_{ij}$ for all $i \in [K]$, $l\in [k]$ in $\cO (k K d R_{\max }^2)$ operations, (2) using the recurrence relation in \cref {eq:alpha-recurrence} to compute $B_{k}\left ( \kappa ^{(1)}_{ij}, \dots , \kappa ^{(k)}_{ij} \right )$ for all $i \in [K]$ in $\cO (k^2 K)$ operations. In total, $\nabla _{\pi _j} \phi ^{(k)} (\btheta )$ takes $\cO (k^2 K + k K d R_{\max }^2)$ operations. $\nabla _{{\bmu }_j} \phi ^{(k)} (\btheta )$ requires (1) pre-computing $\kappa ^{(l)}_{ij}$ for all $i \in [K]$, $l\in [k]$ in $\cO (k K d R_{\max }^2)$ operations, (2) pre-computing $\nabla _{{\bmu }_j} \kappa ^{(l)}_{ij}$ for all $i \in [K]$, $l\in [k]$ in $\cO (k K d R_{\max })$ operations, (3) using the recurrence relation in \cref {eq:alpha-recurrence} to compute $B_{k-l}\left (\kappa ^{(1)}_{ij}, \dots , \kappa ^{(k-l)}_{ij} \right ), l=1, \dots ,k$ for all $i \in [K]$ in $\cO (k^2 K)$ operations. In total, $\nabla _{{\bmu }_j} \phi ^{(k)} (\btheta )$ takes $\cO (k^2 K + k K d R_{\max }^2)$ operations. With a similar calculation, $\nabla _{V_j}\phi ^{(k)} (\btheta )$ takes $\cO (k^2 K + k K d R_{\max }^2)$ operations. \space \end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndv}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofv{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndv}]\phantomsection\label{proof:prAtEndv}\label {pf:computational-complexity-inner} We compute $\psi ^{(k)} (\btheta ; \by _{n})$ by applying \cref {prop:mom-cum-bell}: \begin {align} \psi ^{(k)} (\btheta ; \by _{n}) = \sum _{j=1}^K \pi _j \left \langle \cM ^{(k)}({\btheta }_j), {\by _n}^{\otimes k}\right \rangle = \sum _{j=1}^K \pi _j B_{k}\left ({{\by _n}}^\top {\bmu }_j, {{\by _n}}^\top V_j {V_j}^\top {\by _n}, 0, \dots , 0\right ).\label {eq:F_2} \end {align} The Bell polynomials are evaluated by applying the recurrence relation: \begin {align} \label {eq:beta-recurrence} \begin {cases*} B_0 = 1, & (base case)\\ B_{1}\left ({{\by _n}}^\top {\bmu }_j, {{\by _n}}^\top V_j {V_j}^\top {\by _n}, 0, \dots , 0\right ) = {{\by _n}}^\top {\bmu }_j, & (base case) \\ B_{k}\left ({{\by _n}}^\top {\bmu }_j, {{\by _n}}^\top V_j {V_j}^\top {\by _n}, 0, \dots , 0\right ) = \\ \quad B_{k-1}\left ({{\by _n}}^\top {\bmu }_j, {{\by _n}}^\top V_j {V_j}^\top {\by _n}, 0, \dots , 0\right ) {{\by _n}}^\top {\bmu }_j \\ \quad + (k-1) B_{k-2}\left ({{\by _n}}^\top {\bmu }_j, {{\by _n}}^\top V_j {V_j}^\top {\by _n}, 0, \dots , 0\right ) {{\by _n}}^\top V_j {V_j}^\top {\by _n}. & (induction step) \end {cases*} \end {align} Using \cref {eq:F_2}, the chain rule, and the derivative of the Bell polynomials, we compute $\nabla _{\pi _j} \psi ^{(k)} (\btheta ; \by _{n})$, $\nabla _{{\bmu }_j} \psi ^{(k)} (\btheta ; \by _{n}), \nabla _{V_j} \psi ^{(k)} (\btheta ; \by _{n})$ for each $j$-th component: \begin {align} \nabla _{\pi _j}\psi ^{(k)} (\btheta ; \by _{n}) &= B_{k}\left ({{\by _n}}^\top {\bmu }_j, {{\by _n}}^\top V_j {V_j}^\top {\by _n}, 0, \dots , 0\right ), \\ \nabla _{{\bmu }_j} \psi ^{(k)} (\btheta ; \by _{n}) &= k \pi _j B_{k-1}\left ({{\by _n}}^\top {\bmu }_j, {{\by _n}}^\top V_j {V_j}^\top {\by _n}, 0, \dots , 0\right ) {\by _n}, \\ \nabla _{V_j} \psi ^{(k)} (\btheta ; \by _{n}) &= \begin {cases*} 0, & ($k = 1$)\\ 2 \binom {k}{2} \pi _j B_{k-2}\left ({{\by _n}}^\top {\bmu }_j, {{\by _n}}^\top V_j {V_j}^\top {\by _n}, 0, \dots , 0\right ){\by _n} {{\by _n}}^\top V_j, & ($k \geq 2)$. \end {cases*} \end {align} For all $j\in [K]$, ${{\by _n}}^\top {\bmu }_j$, and ${{\by _n}}^\top V_j {V_j}^\top {\by _n}; \by _n {{\by _n}}^\top V_j$ can be pre-computed in $\cO (K d)$, $\cO (K dR_{\max })$, and $\cO (K dR_{\max })$, respectively, by carefully choosing the order of matrix multiplication. For all $j \in [K]$, using the recurrence relation in \cref {eq:beta-recurrence}, we can compute $B_{k}\left ({{\by _n}}^\top {\bmu }_j, {{\by _n}}^\top V_j {V_j}^\top {\by _n}, 0, \dots , 0\right )$ in $\cO (k K)$ operations. In total, $\psi ^{(k)} (\btheta ; \by _{n})$, $\nabla _{\pi _j} \psi ^{(k)} (\btheta ; \by _{n})$, $\nabla _{{\bmu }_j} \psi ^{(k)} (\btheta ; \by _{n})$, and $\nabla _{V_j} \psi ^{(k)} (\btheta ; \by _{n})$ each requires $\cO (k K + K dR_{\max })$ operations. \space \end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvi}]\phantomsection\label{proof:prAtEndvi}\label {pf:computational-complexity-inner-prod-sum} The sum $\sum _{n^\prime } C_{k,n,n^\prime }$ can be approximated in the following steps: \begin {enumerate} \item Select $m$ landmarks from $N$ points using $k$-means++ sampling proposed in \cite {oglic2017nystrom}, which takes $\cO (Nd m)$ operations ($d$-dimensional distances for $N$ points for $m$ centroids). \item Compute $C^{(k)}$, an $N$-by-$m$ matrix containing kernel evaluations between all $N$ data points and the $m$ landmarks, which takes $\cO (N d m)$ operations. \item Compute $W^{(k)}$, an $m$-by-$m$ Gram matrix on the $m$ landmarks for the $k$-th order moment, which takes $\cO (m^2 d)$ operations. \item Apply pivoted Cholesky decomposition to factorize $W^{(k)} \approx L^{(k)} \left (L^{(k)}\right )^\top $, where $L^{(k)}$ is the Cholesky factor of rank $R_{\text {Chol}} < m$. This takes $\cO \left (m R_{\text {Chol}}^2\right )$ operations. \item To compute the inverse $\left (W^{(k)}\right )^{-1} \bv $ (which is required for the Nyström approximation), we perform a forward and back substitution through the triangular factor: $L^{(k)} \bz = \bv $ (forward substitution) and then $\left (L^{(k)}\right )^\top \by = \bz $ (back substitution). This step takes $\cO (m^2)$ operations. \item After obtaining the solution vector $\by $ from the triangular solve step, we compute the approximate $\sum _{n^\prime }C_{k,n,n^\prime } \approx C^{(k)} \by $, which takes $\cO (N m)$ operations. \item [] Thus, the overall computational complexity is $\cO \left (Ndm + m^2 d + mR_{\text {Chol}}^2 + m^2 + Nm \right )$. Taking the dominant terms, we get $\cO \left (Ndm\right )$. \end {enumerate}\end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndvii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofvii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndvii}]\phantomsection\label{proof:prAtEndvii}\label {pf:approximation-error-kernel} Applying \cite [Theorem~5]{oglic2017nystrom} to our problem, we get \begin {align} \label {ineq:fraction-error-bound} \EX \left [\frac {\norm {H^{(k)} - \widetilde {H^{(k)}_m}}_F}{\norm {H^{(k)} - H^{(k)}_m}_F}\right ] &\leq 8\left (\ln (m+1)+2\right ) \left (\sqrt {N - m}+ \frac {\phi (C^\star \mid U_{m})}{ \norm {H^{(k)}- H^{(k)}_m}_F}\right ). \end {align} \par Under polynomial spectral decay of $H^{(k)}$, $\lambda _i^{(k)} \in \cO (i^{-a})$ with $a>1$, i.e., there exists some constant $C > 0$ such that for large $i$, $\lambda _i^{(k)} \leq C i^{-a}$ for $a>1$. By the integral test, we have \begin {align*} \norm {H^{(k)}-H^{(k)}_{m}}_F^2 = \sum _{i= m+1}^{N}\left (\lambda _{i}^{(k)}\right )^2 &\leq \sum _{i= m+1}^{N}\left (C i^{-a}\right )^2 \leq C^2 \int _{m}^{N} x^{-2a} \mathrm {d}x\\ &= \frac {C^2}{2a-1}\left (m^{-2a+1} - N^{-2a+1}\right ) \leq \frac {C^2}{2a-1}\left (m^{-2a+1}\right ). \end {align*} \par After taking the square root on both sides, we get $\norm {H^{(k)}-H^{(k)}_{m}}_F \leq \frac {C}{\sqrt {2a-1}}\left (m^{-a+1/2}\right )$. Combining this, \cref {ineq:fraction-error-bound}, and the cluster potential condition in \cref {ineq:cluster-aligned-condition}, we get \begin {align*} \EX \left [\norm {H^{(k)} - \widetilde {H^{(k)}_m}}_F\right ] &\leq 8\left (\ln (m+1)+2\right ) \left (\sqrt {N - m} \norm {H^{(k)}- H^{(k)}_m}_F + \phi (C^\star \!\mid U_{m})\right )\\ &\leq 8 \left (\ln (m+1)+2\right ) \left (2\sqrt {N - m} \norm {H^{(k)}- H^{(k)}_m}_F\right )\\ &\leq 16 \left (\ln (m+1)+2\right ) \sqrt {N - m} \frac {C}{\sqrt {2a-1}}\left (m^{-a+1/2}\right ),\\ \text {which implies that } & \EX \left [\norm {H^{(k)}-\widetilde {H^{(k)}_{m}}}_{F}\right ] \in \cO \left (\ln (m) \sqrt {N- m}\left (m^{-a+1/2}\right )\right ). \text { In particular, } \\ \text {as } m \to \rank H^{(k)}, \text { }& \text {the expected error goes to zero.} \end {align*}\end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndviii}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofviii{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndviii}]\phantomsection\label{proof:prAtEndviii}\label {pf:rank-algebraic-bound} Since $\by _{1},\dots ,\by _{N} \iid $ \cref {model:heteroscedastic}, by the characterization of its distribution given in \cref {prop:pdf-single-gaussian-lowrank}, $\by _{1},\dots ,\by _{N}$ lie in a union of $K$ affine subspaces, $\bigcup _{j=1}^{K} U_{j}, \quad \dim U_{j}=R_{j}\leq R_{\max }.$ Every point $\by \in U_{j} = \bmu _j + \range (\Sigma _j)$ lies in the linear subspace $\text {span}\{\bmu _j\} + \range (\Sigma _j) $, whose dimension is at most $R_j + 1$. Writing $\by $ in a basis of this subspace, every coordinate of $\by ^{\otimes k}$ is then a homogeneous polynomial of degree $k$ in at most $R_j + 1$ variables. Since the number of distinct monomials of degree $k$ in $R_j + 1$ variables is $\binom {R_j+k}{k}$, $\by ^{\otimes k}$ with $\by \in U_j$ span at most $\binom {R_j+k}{k}$ directions. \par The global span is therefore contained in the sum of these $K$ subspaces, with dimension bounded by $\sum _{j=1}^{K}\binom {R_{j}+k}{k}$. Then, $\rank H^{(k)} \leq \sum _{j=1}^{K}\binom {R_{j}+k}{k} \leq K \binom {R_{\max }+k}{k}$. If we further assume that $U_j$ is contained in a single linear subspace $U$ with $\dim U \leq R_{\max }$ for all $j$, then all observations lie in the linear subspace $U$ itself. In this case, we would not need the additional dimension for $\bmu _j$, and $\by ^{\otimes k}$ span at most $\binom {\dim U+k-1}{k} \leq \binom {R_{\max }+k-1}{k}$ directions.\end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndix}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofix{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndix}]\phantomsection\label{proof:prAtEndix}\label {pf:computational-complexity-W} The numerator of $\widehat {w}_k^{[t]}$ in \cref {eq:d-gmom-multistep} can be written as \begin {equation*} \begin {split} &\sum _{i \in \cI _k} \widehat {S}^{[t]}_{ii} = \sum _{i \in \cI _k} \left (\frac {1}{N}\sum _{n=1}^{N} g(\widehat {{\btheta }}^{[t-1]}; \by _n) g(\widehat {{\btheta }}^{[t-1]}; \by _n)^\top \right )_{ii} = \sum _{i \in \cI _k}\frac {1}{N} \sum _{n=1}^{N} g(\widehat {{\btheta }}^{[t-1]}; \by _n)_i^2\\ &= \frac {1}{N} \sum _{n=1}^{N} \norm {\vectorize {\left (\cM ^{(k)}\left (\widehat {{\btheta }}^{[t-1]}\right ) - {\by _n}^{\otimes k}\right )}}^2 = \frac {1}{N} \sum _{n=1}^{N} \norm {\cM ^{(k)}\left (\widehat {{\btheta }}^{[t-1]}\right ) - {\by _n}^{\otimes k}}^2\\ &= \frac {1}{N} \sum _{n=1}^{N} \norm {\cM ^{(k)}\left (\widehat {{\btheta }}^{[t-1]}\right )}^2 - 2 \inner {\cM ^{(k)}\left (\widehat {{\btheta }}^{[t-1]}\right )}{{\by _n}^{\otimes k}} +\inner {{\by _n}}{{\by _n}}^k. \end {split} \end {equation*} The denominator of $\widehat {w}_k^{[t]}$ in \cref {eq:d-gmom-multistep} can be written as \begin {equation*} \begin {split} &\sum _{i \in \cI _k}\sum _{j=1}^{q} \left (\widehat {S}^{[t]}_{ij}\right )^2 = \sum _{i \in \cI _k}\sum _{j=1}^{q} \left (\frac {1}{N}\sum _{n=1}^{N} g(\widehat {{\btheta }}^{[t-1]}; \by _n) g(\widehat {{\btheta }}^{[t-1]}; \by _n)^\top \right )_{ij}^2\\ &= \frac {1}{N^2}\sum _{n,n^\prime =1}^{N} \sum _{i \in \cI _k} \left (\sum _{j=1}^{q}\left (g(\widehat {{\btheta }}^{[t-1]}; \by _n) g(\widehat {{\btheta }}^{[t-1]}; \by _n)^\top \right )_{ij} \left (g(\widehat {{\btheta }}^{[t-1]}; \by _{n^\prime }) g(\widehat {{\btheta }}^{[t-1]},\by _{n^\prime })^\top \right )_{ij} \right )\\ = &\frac {1}{N^2}\sum _{n,n^\prime =1}^{N} \inner {g(\widehat {{\btheta }}^{[t-1]}; \by _n)[i_k:{i_k}^{\prime }]}{g(\widehat {{\btheta }}^{[t-1]}; \by _{n^\prime })[i_k:{i_k}^{\prime }]} \Tr (g(\widehat {{\btheta }}^{[t-1]}; \by _n)g(\widehat {{\btheta }}^{[t-1]}; \by _{n^\prime })^\top )\\ = &\frac {1}{N^2}\sum _{n,n^\prime =1}^{N} \inner {g(\widehat {{\btheta }}^{[t-1]}; \by _n)[i_k:{i_k}^{\prime }]}{g(\widehat {{\btheta }}^{[t-1]}; \by _{n^\prime })[i_k:{i_k}^{\prime }]} \Tr (g(\widehat {{\btheta }}^{[t-1]}; \by _{n^\prime })^\top g(\widehat {{\btheta }}^{[t-1]}; \by _n))\\ = &\frac {1}{N^2}\sum _{n,n^\prime =1}^{N} \inner {g(\widehat {{\btheta }}^{[t-1]}; \by _n)[i_k:{i_k}^{\prime }]}{g(\widehat {{\btheta }}^{[t-1]}; \by _{n^\prime })[i_k:{i_k}^{\prime }]} \inner {g(\widehat {{\btheta }}^{[t-1]}; \by _n))}{g(\widehat {{\btheta }}^{[t-1]}; \by _{n^\prime })}\\ = &\frac {1}{N^2}\sum _{n,n^\prime =1}^{N} \inner {\cM ^{(k)}\left (\widehat {{\btheta }}^{[t-1]}\right ) - {\by _n}^{\otimes k }}{\cM ^{(k)} - \by _{n^\prime }^{\otimes k }} \sum _{k^\prime =1}^L \inner {\cM ^{(k^\prime )}\left (\widehat {{\btheta }}^{[t-1]}\right ) - {\by _n}^{\otimes k^\prime }}{\cM ^{(k^\prime )} - \by _{n^\prime }^{\otimes k^\prime }} \end {split} \end {equation*} Combining the numerator and the denominator, substituting with the quantities in \cref {eq:alpha-beta-gamma}, and simplifying, we get the expression for DGMM weights in \cref {eq:w_k}. Observe that $\widehat {w}^{[t]}_k$ requires (1) $\phi _k^{[t-1]} = \norm {\cM ^{(k)}\left (\widehat {{\btheta }}^{[t-1]}\right )}^2, k = 1, \dots , L,$ which, by \cref {thm:computational-complexity-norm}, takes $\cO (L^2 K^2 + L K^2 d R_{\max }^2)$ operations, and (2) $\psi _{k,n}^{[t-1]} = \inner {\cM ^{(k)}\left (\widehat {{\btheta }}^{[t-1]}\right )}{\by _{n}^{\otimes k}}$, $k = 1, \dots , L, n = 1, \dots , N,$ which, by \cref {thm:computational-complexity-inner}, takes $\cO (NLK + NKdR_{\max })$ operations. In total, $\widehat {w}^{[t]}_k$ in \cref {eq:d-gmom-multistep} can be computed in $\cO (L^2 K^2 + L K^2 d R_{\max }^2 + NLK + NKdR_{\max })$. \space \end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndx}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofx{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndx}]\phantomsection\label{proof:prAtEndx}\label {pf:computational-complexity-gradients} We rewrite the DGMM objective function in \cref {eq:d-gmom-multistep}: \begin {align*} Q^{[t]}_N(\btheta ) &= \overline {g}_N\left ({\btheta }\right )^\top \diag (\underbrace {\widehat {w}^{[t]}_1, \dots , \widehat {w}^{[t]}_1}_{d \text { copies}}, \dots , \underbrace {\widehat {w}^{[t]}_L, \dots , \widehat {w}^{[t]}_L}_{d^L \text { copies}}) \overline {g}_N\left ({\btheta }\right )\\ =&\sum _{k=1}^L \widehat {w}^{[t]}_k \sum _{i \in \cI _k} \left (\vectorize \left (\cM ^{(k)}\left ({\btheta }\right )- \frac {1}{N} \sum _{n=1}^N {\by _n}^{\otimes k }\right )_i\right )^2=\sum _{k=1}^L \widehat {w}^{[t]}_k \norm {\cM ^{(k)}\left ({\btheta }\right ) - \frac {1}{N} \sum _{n=1}^N {\by _n}^{\otimes k }}^2\\ =&\sum _{k=1}^L \widehat {w}^{[t]}_k \left (\norm {\cM ^{(k)}\left ({\btheta }\right )}^2 - \frac {2}{N} \sum _{n=1}^N\left \langle \cM ^{(k)} \left ({\btheta }\right ), {\by _n}^{\otimes k}\right \rangle + \frac {1}{N^2}\sum _{n=1}^N \sum _{n^{\prime }=1}^N \left \langle {\by _n}^{\otimes k}, \by _{n^{\prime }}^{\otimes k}\right \rangle \right ),\\ =&\sum _{k=1}^L \widehat {w}^{[t]}_k \left (\phi ^{(k)} (\btheta ) - \frac {2}{N} \sum _{n=1}^N \psi ^{(k)} (\btheta ; \by _{n}) + \frac {1}{N^2}\sum _{n=1}^N \sum _{n^{\prime }=1}^N C_{k,n,n^\prime }\right ).\numberthis \label {eq:gmm-objective-rewrite} \end {align*} Observe that $\nabla _{{\btheta }} Q^{[t]}_N(\btheta )$ requires the following gradients: $\nabla _{\pi _j}\phi ^{(k)} (\btheta ), \nabla _{{\bmu }_j}\phi ^{(k)} (\btheta ), \mkern 9mu \nabla _{V_j} \phi ^{(k)} (\btheta )$ and $\nabla _{\pi _j} \psi ^{(k)} (\btheta ; \by _{n}), \nabla _{{\bmu }_j} \psi ^{(k)} (\btheta ; \by _{n}), \nabla _{V_j} \psi ^{(k)} (\btheta ; \by _{n})$, for $k = 1, \dots , L, n = 1, \dots , N$, which, by \cref {thm:computational-complexity-norm} and \cref {thm:computational-complexity-inner}, takes $\cO (L^2 K^2 + LK^2 dR_{\max }^2 + NLK + NKdR_{\max })$ operations in total. $\nabla _{{\btheta }} Q^{[t]}_N(\btheta )$ is then obtained by vectorizing and concatenating these gradients. \par \space \end{proof}

\makeatletter\Hy@SaveLastskip\label{proofsection:prAtEndxi}\ifdefined\pratend@current@sectionlike@label\immediate\write\@auxout{\string\gdef\string\pratend@section@for@proofxi{\pratend@current@sectionlike@label}}\fi\Hy@RestoreLastskip\makeatother\begin{proof}[Proof of \pratendRef{thm:prAtEndxi}]\phantomsection\label{proof:prAtEndxi}\label {pf:computational-complexity-comparison} Let $I$ be the number of L-BFGS iterations, $T$ the number of GMM steps. The DGMM estimator, $\widehat {\btheta }^{(\dgmm )}$, requires the following computations: \begin {enumerate} \item For one time, pre-compute $\sum _{n^\prime = 1}^N C_{k,n,n^\prime }, \text { for } k = 1, \dots , 2L, n = 1, \dots , N,$ and store in a $(2L+1)\times N$ matrix. By \cref {thm:computational-complexity-inner-prod-sum}, this requires $\cO (NLdm)$ operations. \item For at most $T$ times, compute $\widehat {w}_k^{[t-1]}$ for $k = 1, \dots , L$, which, by \cref {thm:computational-complexity-W}, takes $\cO (T L^2 K^2 + T L K^2 d R_{\max }^2 + T NLK + T NKdR_{\max })$ operations. \item For at most $I$ times, compute the necessary gradients, which, by \cref {thm:computational-complexity-gradients}, takes $\cO (I L^2 K^2 + I L K^2 dR_{\max }^2 + I NLK + I NKdR_{\max })$ operations. \end {enumerate} Taking the dominant terms and absorbing the stopping criteria constants, we get that the overall computational complexity of the DGMM estimator ${{\widehat {\btheta }}^{(\dgmm )}}$ in \cref {eq:d-gmom-multistep} is $\cO (L^2 K^2 + L K^2 dR_{\max }^2 + NLK + NKdR_{\max } + NLdm)$. \par In contrast, the MM estimator, ${\widehat {\btheta }}^{(\mm )}$, requires the following computations: \begin {enumerate} \item For one time, pre-compute the sample moments, which takes $\cO (Nq)$, where $q = d + d^2 + \cdots + d^L$. Taking the dominant terms, we get $\cO (N d^{L})$. \item The weighting matrix is the identity matrix and therefore takes $\cO (1)$ time to compute. \item For at most $I$ times, compute the moment condition vector $\overline {g}_N(\btheta )$ in $\cO (Nq)$ operations, the objective function $\overline {g}_N(\btheta )^\top \overline {g}_N(\btheta )$ in $\cO (q^2)$ operations, the Jacobian matrix $G(\btheta ) = \frac {\partial \overline {g}_N(\btheta )}{\partial \btheta } \in \R ^{q\times p}$ in $\cO (Nqp)$ operations, and the gradients $\nabla _{\btheta } \overline {g}_N(\btheta )^\top \overline {g}_N(\btheta ) = 2 G(\btheta )^\top \overline {g}_N(\btheta )$ in $\cO (qp)$ operations. Taking the dominant term and absorbing the stopping criteria constants, we get $\cO (INd^{L+1}KR_{\max }+ Id^{L+1}K R_{\max }) = \cO (Nd^{L+1}KR_{\max })$. \end {enumerate} \par Similarly, the GMM estimator, ${\widehat {\btheta }}^{(\gmm )}$, requires the following computations: \begin {enumerate} \item For one time, pre-compute the sample moments, which takes $\cO (N q)$. \item For at most $T$ times, compute $\widehat {S}^{[t]}$ in $\cO (N q^2)$ and invert $\widehat {S}^{[t]}$ in $\cO (q^3)$. \item For at most $I$ times, compute the moment condition vector $\overline {g}_N(\btheta )$ in $\cO (Nq)$ operations, the objective function $\overline {g}_N(\btheta )^\top \widehat {W}^{[t]}\overline {g}_N(\btheta )$ in $\cO (q^2)$ operations, the Jacobian matrix $G(\btheta ) = \frac {\partial \overline {g}_N(\btheta )}{\partial \btheta }$ in $\cO (Nqp)$ operations, and the gradients $\nabla _{\btheta } \overline {g}_N(\btheta )^\top \widehat {W}^{[t]} \overline {g}_N(\btheta ) = 2 G(\btheta )^\top \widehat {W}^{[t]} \overline {g}_N(\btheta )$ in $\cO (q^2 p)$ operations. Taking the dominant term, we get $\cO (INd^{L+1}KR_{\max }+ Id^{2L+1}K R_{\max })$. \item The overall computational complexity of obtaining ${{\widehat {\btheta }}^{(\gmm )}}$ is $\cO (Nd^{2L} + d^{3L} + Nd^{L+1}KR_{\max }+ d^{2L+1}K R_{\max })$ after absorbing the stopping criteria constants. \end {enumerate} \par \end{proof}

